A Simple Recipe for Competitive Low-compute Self supervised Vision Models

Self-supervised methods in vision have been mostly focused on large architectures as they seem to suffer from a significant performance drop for smaller architectures. In this paper, we propose a simple self-supervised distillation technique that can train high performance low-compute neural networks. Our main insight is that existing joint-embedding based SSL methods can be repurposed for knowledge distillation from a large self-supervised teacher to a small student model. Thus, we call our method Replace one Branch (RoB) as it simply replaces one branch of the joint-embedding training with a large teacher model. RoB is widely applicable to a number of architectures such as small ResNets, MobileNets and ViT, and pretrained models such as DINO, SwAV or iBOT. When pretraining on the ImageNet dataset, RoB yields models that compete with supervised knowledge distillation. When applied to MSN, RoB produces students with strong semi-supervised capabilities. Finally, our best ViT-Tiny models improve over prior SSL state-of-the-art on ImageNet by $2.3\%$ and are on par or better than a supervised distilled DeiT on five downstream transfer tasks (iNaturalist, CIFAR, Clevr/Count, Clevr/Dist and Places). We hope RoB enables practical self-supervision at smaller scale.

==> tables/deprecated/ablation_multicrop.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{c c|c c c}
        Method & Teacher & IN1K & IN1k 1\% & iNat18 \\
        \midrule
        RoB (300ep) & DINO S/8 & 71.4 & 54.0 & 39.8 \\
        \ac \textbf{w/o} multi-crop & DINO S/8 & 70.4 & 53.4 & 35.4 \\
        \bottomrule
    \end{tabular}
    \caption{\textbf{Multi-crop is needed get the best results} in-distribution and in transfer tasks. In particular on iNaturalist18, the gap is very significant, reaching almost $5\%$.}
    \label{tab:ablation_multicrop}
\end{table}

==> tables/deprecated/ablation_swapped.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{c c|c c c}
        Method & Teacher & IN1K & IN1k 1\% & iNat18 \\
        \midrule
        RoB (300ep) & DINO S/8 & 71.4 & 54.0 & 39.8 \\
        \ac w/i cross-view & DINO S/8 & 71.4 & 54.0 & 39.4 \\
        \midrule
        RoB (300ep) & iBOT L/16 & 71.8 & 56.2 & 37.4 \\
        \ac w/i cross-view & iBOT L/16 & 71.7 & 55.9 & 36.5 \\
        \bottomrule
    \end{tabular}
    \caption{\textbf{Identical-view assignment} is beneficial compared to cross-view assignments.}
    \label{tab:ablation_swapped}
\end{table}

==> tables/deprecated/dino_to_rn.tex <==
\begin{table*}[]
    \centering
    \begin{tabular}{c|c c|c c c c c c | c}
        Student & Teacher & Params & IN1k & iNat18 & Clevr/C & Clevr/D & Cifar100 & Places205 & Mean \\
        \midrule
        \multirow{2}{*}{RN18}
        & SwAV RN50 & 24M & 66.7 & 37.2 & \bf 73.0 & \bf 66.5 & \bf 69.2 & \bf 49.5 & 60.35 \\
        & DINO S/8 & 22M & \bf 68.3 & \bf  41.0 & \bf 72.8 & 64.7 & 68.1 & 48.0 & \bf 60.48 \\
        \midrule
        \multirow{2}{*}{RN34}
        & SwAV RN50 & 24M & 70.4 & 39.5 & 73.6 & \bf 66.3 & \bf 73.7 & \bf 51.1 & 62.43 \\
        & DINO S/8 & 22M & \bf 72.6 & \bf 43.7 & \bf 74.2 & 65.1 & 72.1 & 50.8 & \bf 63.08 \\
        \bottomrule
    \end{tabular}
    \caption{Cross architecture self-supervised distillation. Self supervised vision transformer show strong performance in distribution and on transfer benchmarks such as iNaturalist. Self-supervised distillation allows to benefit from those strong baselines to improve ResNet self-supervised baselines.}
    \label{tab:dino_to_rn}
\end{table*}

==> tables/deprecated/scaling_teachers.tex <==
\begin{table*}[]
    \centering
    \begin{tabular}{c|c c|c c c c c c | c}
        Student & Teacher & Params & IN1K & iNat18 & Clevr/C & Clevr/D & Cifar100 & Places205 & Mean \\
        \midrule
        RN18 & SwAV RN50 & 24M & 66.7 & 37.2 & 73.0 & 66.5 & 69.2 & 49.5 & 60.35\\
        RN18 & SwAV RG128 & 638M & 67.4 & 37.5 & 72.2 & 67.3 & 69.0 & 49.3 & \bf 60.45 \\
        % RN18 & $\Delta$ & & +0.7 & +0.3 & -0.8 & +0.8 & -0.2 & -0.2 & +0.10 \\
        \midrule
        RN34 & SwAV RN50 & 24M & 70.4 & 39.5 & 73.6 & 66.3 & 73.7 & 51.1 & 62.43\\
        RN34 & SwAV RG 128 & 638M & 71.3 & 40.3 & 72.6 & 65.9 & 73.9 & 51.3 & \bf 62.55 \\
        % RN34 & $\Delta$ & & +0.9 & +0.8 & -1.0 & -0.4 & +0.2 & +0.2 & +0.12\\
        \midrule
        ViT/T16 & iBOT B/16 & 86M & 71.4 & 36.9 & 81.3 & 65.1 & 75.7 & 49.1 & 63.25 \\
        ViT/T16 & iBOT L/16 & 303M & 71.8 & 37.4 & 81.3 & 66.0 & 76.8 & 49.6 & \bf 63.82 \\
        % ViT/T16 & $\Delta$ & & +0.4 & +0.5 & -0.0 & +0.9 & +1.1 & +0.5 & +0.57 \\
        \bottomrule
    \end{tabular}
    \caption{Effect of scaling teachers on the performance of the student. All students are trained for 300 epochs. Using a stronger iBOT teacher improves overall performance. On ResNets, using a strong RegNet128Gf teacher improves high level semantic transfer tasks.}
    \label{tab:scaling_teachers}
\end{table*}

==> tables/deprecated/vs_dist_kd.tex <==
\begin{table*}[]
    \centering
    \begin{tabular}{c|c c|c c c c c c | c}
        Arch & Method & Teacher & IN1K & iNat18 & Clevr/C & Clevr/D & Cifar100 & Places205 & Mean \\
        \hline
        \hline
        RN18 & RNSB A1 & \quentin{to gray} & \bf 71.5 & 35.2 & 59.5 & 61.7 & 69.0 & 46.5 & 57.23 \\
        RN18 & DIST\_KD & RN50 SB A1 & 74.3 & \bf 37.6 & 58.8 & 59.6 & \bf 72.2 & 47.4 & 58.31 \\
        \hline
        RN18 & Ours SwAV & SwAV RN50 & 66.7 & 37.2 & \bf 73.0 & \bf 66.5 & 69.2 & \bf 49.5 & \bf 60.35 \\
        RN18 & $\Delta$ & - & -7.6 & -0.4 & +14.2 & +6.9 & -3.0 & +2.1 & +2.04 \\
        \hline
        \hline
        RN34 & RNSB A1 & \quentin{to gray} & 76.3 & 36.2 & 56.8 & 59.9 & 71.4 & 48.1 & 58.12 \\
        RN34 & DIST\_KD & RN50 SB A1 & \bf 77.8 & 36.6 & 56.2 & 58.6 & \bf 73.9 & 48.8 & 58.65 \\
        \hline
        RN34 & Ours & SwAV RN50 & 70.4 & \bf 39.5 & \bf 73.6 & \bf 66.3 & 73.7 & \bf 51.1 & \bf 62.43\\
        RN34 & $\Delta$ & - & -7.4 & +2.9 & +17.4 & +7.7 & -0.2 & +1.3 & + 3.78 \\
        \hline
        \hline
        ViT/T16 & DEIT & \quentin{to gray} & \bf 72.2 & 36.3 & 67.2 & 54.1 & 73.5 & 48.1 & 58.57 \\
        ViT/T16 & DEIT & RegNet16Gf & \bf 74.5 & 38.1 & 70.7 & 56.7 & 74.8 & 48.6 & 60.57 \\
        \hline
        ViT/T16 & Ours & DINO S/8 & 71.4 & \bf 39.8 & 79.8 & 62.9 & \bf 77.1 & 48.4 & 63.23 \\
        ViT/T16 & $\Delta$ & & -3.1 & +1.7 & +9.1 & +6.2 & +2.3 & -0.2 & +2.66 \\
        \hline
        ViT/T16 & Ours & iBOT L/16 & 71.8 & 37.4 & \bf 81.3 & \bf 66.0 & \bf 76.8 & \bf 49.6 & \bf 63.82 \\
        ViT/T16 & $\Delta$ & & -2.7 & -0.7 & +10.6 & +9.3 & +2.0 & +1.0 & +3.25 \\
        \hline
        \hline
    \end{tabular}
    \caption{Comparing the transfer performance of self-supervised distillation against the same model distilled in a supervised way using DIST\_KD, one the strongest supervised distillation methods, on a strong ResNet50 Strikes Back teacher.}
    \label{tab:vs_dist_kd}
\end{table*}
